Decision Variance in Online Learning

Online learning has traditionally focused on the expected rewards. In this paper, a risk-averse online learning problem under the performance measure of the mean-variance of the rewards is studied. Both the bandit and full information settings are considered. The performance of several existing policies is analyzed, and new fundamental limitations on risk-averse learning is established. In particular, it is shown that although a logarithmic distribution-dependent regret in time $T$ is achievable (similar to the risk-neutral problem), the worst-case (i.e. minimax) regret is lower bounded by $\Omega(T)$ (in contrast to the $\Omega(\sqrt{T})$ lower bound in the risk-neutral problem). This sharp difference from the risk-neutral counterpart is caused by the the variance in the player's decisions, which, while absent in the regret under the expected reward criterion, contributes to excess mean-variance due to the non-linearity of this risk measure. The role of the decision variance in regret performance reflects a risk-averse player's desire for robust decisions and outcomes.

==> ProofThm2.tex <==
\begin{proof}[Proof of Theorem~\ref{Thm2}]

Let $[T]=\{1,2,\dots,T\}$ denote the set of time instances. For each $S\subseteq [T]$ and any policy $\pi$ in a 2-armed bandit, we construct a new policy $\pi^{S}$, based on $\pi$, that is obtained by altering the decision of policy $\pi$ on set $S$. In particular,
\begin{eqnarray}
\begin{cases}
&\pi^{S}_t = \pi_t,~~\text{if}~t\not\in S\\
&\pi^{S}_t = 3-\pi_t,~~\text{if}~t\in S.\\
\end{cases}
\end{eqnarray}

In a 2-armed bandit, let $\Delta=\Delta_k$ where $k\in\{1,2\}$ and $k\neq*$. 
In the second term in regret expression given in~\eqref{RegUB}, we have
\begin{eqnarray}\nn
&&\hspace{-5em}\E_\F\left[\left(\sum_{\substack{k=1 \\k\neq k^*}}^K (\I[\pi_{t}=k]-\Pr_\F[\pi_{t}=k])\Delta_k\right)^2\right]\\\nn 
&=& 
\E_\F\left[\left( (\I[\pi_{t}\neq*]-\Pr_\F[\pi_{t}\neq*])\Delta\right)^2\right]\\\nn
&=&\Pr_\F[\pi_{t}\neq*](1-\Pr_\F[\pi_{t}\neq*])\Delta^2.
\end{eqnarray}
The first term in the regret expression given in~\eqref{RegUB}, is always positive. Thus
\begin{eqnarray}\label{Seq0}
\Reg_{\F}(T)\ge \sum_{t=1}^T \Pr_\F[\pi_{t}\neq*](1-\Pr_\F[\pi_{t}\neq*])\Delta^2.
\end{eqnarray}

Since $\pi_t^S = \pi_t$ or $1-\pi_t$, we have, for all $S\subseteq[T]$
\begin{eqnarray}\label{Seq1}
\Pr_\F[\pi^S_{t}\neq*](1-\Pr_\F[\pi^S_{t}\neq*])\Delta^2 = \Pr_\F[\pi_{t}\neq*](1-\Pr_\F[\pi_{t}\neq*])\Delta^2.
\end{eqnarray}
By construction of $\{\pi^S\}_{S\subseteq[T]}$, there exists a $S_0\subseteq[T]$ that $\Pr_\F[\pi^{S_0}_{t}\neq*]\le\frac{1}{2}$ for all $t\in[T]$. For $S_0$, we have
\begin{eqnarray}\nn
&&\hspace{-3em}\sum_{t=1}^T\Pr_\F[\pi^{S_0}_{t}\neq*](1-\Pr_\F[\pi^{S_0}_{t}=2])\Delta^2\\\label{Sineq1}
&\ge&\frac{1}{2}\sum_{t=1}^T \Pr_\F[\pi^{S_0}_{t}\neq*]\Delta^2.
\end{eqnarray}

From Theorem~\ref{Thm1}, there exists a distributing $\F$ for a 2-armed bandit where 
\begin{eqnarray}\label{Sineq2}
\sum_{t=1}^T\Pr_\F[\pi^{S_0}_t\neq *] \ge \{\frac{0.01}{\Gamma^2}\wedge\frac{T}{2e}\}.
\end{eqnarray}

Thus, combining~\eqref{Seq0},~\eqref{Seq1},~\eqref{Sineq1} and~\eqref{Sineq2}, there exists a distribution $\F$ for a 2-armed bandit where
\begin{eqnarray}\nn
\Reg_\F(T) &\ge& \sum_{t=1}^T \Pr_\F[\pi_{t}\neq*](1-\Pr_\F[\pi_{t}\neq*])\Delta^2\\\nn 
&=&\sum_{t=1}^T \Pr_\F[\pi^{S_0}_{t}\neq*](1-\Pr_\F[\pi^{S_0}_{t}\neq*])\Delta^2\\\nn
&\ge&\frac{1}{2}\sum_{t=1}^T \Pr_\F[\pi^{S_0}_{t}\neq*]\Delta^2\\\nn
&\ge& \{\frac{0.005}{\Gamma^2}\wedge\frac{T}{4e}\}\Delta^2.
\end{eqnarray}

Choosing $\Gamma=\sqrt{\frac{0.02e}{T}}$, we have
\begin{eqnarray}
\Reg_\F(T) \ge \frac{T}{4e}. 
\end{eqnarray}

\end{proof}

==> RegretExp.tex <==
Let $\I[.]$ denote the indicator function that is, for an event $\mathcal{E}$,  $\I[\mathcal{E}]=1$ if and only if $\mathcal{E}$ is true, and $\I[\mathcal{E}]=0$, otherwise. 
Let $\tau_{k,t}=\sum_{s=1}^t\I[\pi_s=k]$ denote the number of times that action $k$ has been chosen until time $t$. 

The risk-neutral regret $\E[ \sum_{t=1}^T (  X_{k_{\max},t}-X_{\pi_t,t}  ) ]$, where $k_{\max}=\argmax_{k\in[K]}\mu_k$, can be expressed as a weighted sum of $\E[\tau_{k,T}]$ with weights $\mu_{k_{\max}}-\mu_k$. In contrast, the risk-averse regret $\Reg(T)$ given in~\eqref{RegretDef} depends also on the variance of the decisions through time. Lemma~\ref{Lemma:RegExp} provides an expression of regret which is used throughout the paper to analyze the performance of the policies. Let $\Gamma_k=\MV_{k}-\MV_{k^*}$ and $\Delta_k=\mu_k-\mu_{k^*}$. Let $\Gamma=\min_{k} \{\Gamma_k:\Gamma_k>0\}$ and $\Gamma_{\max}=\max_{k}\Gamma_k$. 
\begin{lemma}\label{Lemma:RegExp}
The regret of a policy $\pi$ under the measure of total mean-variance of rewards satisfies
\begin{eqnarray}\nn
&&\hspace{-2em}\Reg(T) 
= \sum_{k=1}^K \E[\tau_{k,T}]\Gamma_{k} \\\label{RegUB}
&&\hspace{-1.5em}+\sum_{t=1}^T \E\left[\left(\Sumnotkstar (\I[\pi_{t}=k]-\Pr[\pi_{t}=k])\Delta_k\right)^2\right].~~~~
\end{eqnarray}

\end{lemma}
\emph{Proof.} See Appendix A. 

The regret expression given in Lemma~\ref{Lemma:RegExp} shows that $\Reg(T)\ge0$ for any policy $\pi$, and $R_{\pi^*}(T)=0$ ($\pi^*_t=k^*$), which proves that the optimal single action policy is the optimal policy under the risk-averse measure. The second term in the regret expression in~\eqref{RegUB} captures the variance of the decisions.
